Deep learning based domain adaptation for mitochondria segmentation on EM volumes

Accurate segmentation of electron microscopy (EM) volumes of the brain is essential to characterize neuronal structures at a cell or organelle level. While supervised deep learning methods have led to major breakthroughs in that direction during the past years, they usually require large amounts of annotated data to be trained, and perform poorly on other data acquired under similar experimental and imaging conditions. This is a problem known as domain adaptation, since models that learned from a sample distribution (or source domain) struggle to maintain their performance on samples extracted from a different distribution or target domain. In this work, we address the complex case of deep learning based domain adaptation for mitochondria segmentation across EM datasets from different tissues and species. We present three unsupervised domain adaptation strategies to improve mitochondria segmentation in the target domain based on (1) state-of-the-art style transfer between images of both domains; (2) self-supervised learning to pre-train a model using unlabeled source and target images, and then fine-tune it only with the source labels; and (3) multi-task neural network architectures trained end-to-end with both labeled and unlabeled images. Additionally, we propose a new training stopping criterion based on morphological priors obtained exclusively in the source domain. We carried out all possible cross-dataset experiments using three publicly available EM datasets. We evaluated our proposed strategies on the mitochondria semantic labels predicted on the target datasets. The methods introduced here outperform the baseline methods and compare favorably to the state of the art. In the absence of validation labels, monitoring our proposed morphology-based metric is an intuitive and effective way to stop the training process and select in average optimal models.

==> tables/Att_YNet_parameters_table.tex <==
%\newpage
%\clearpage
%\section{Hyperparameter search for the Attention Y-Net}

%%%%%%%%%%%%%%%%%%%%
%% 1st step table %%
%%%%%%%%%%%%%%%%%%%%

\begin{table}[]
\hspace{-1.4cm}
\begin{adjustbox}{max width=1.22\textwidth}
\begin{tabular}{rcrcr}
\hline
\textbf{Hyperparameter}                                                                                & \phantom{abc}  & \textbf{Search space}                  & \phantom{abc} & \textbf{Best assignment}         \\ \hline
\textbf{Data}                                                                                          & \phantom{abc}  & \phantom{abc}                          & \phantom{abc} & \phantom{abc}                    \\ \hline
Validation                                                                                             &                & True                                   &               & True                             \\
Random validation                                                                                      &                & True                                   &               & True                             \\
\% of train as validation                                                                              &                & 10\%                                   &               & 10\%                             \\
Patches                                                                                                &                & \textit{choice}[Sequential, Random(1000)]           &               & Random(1000)                     \\
Patch size                                                                                             &                & $256\times256$                         &               & $256\times256$                   \\
\begin{tabular}[c]{@{}r@{}}Discard patches with less than \\ a \% of the foreground class\end{tabular} &                & \textit{choice}[True(5\%), True(10\%), False]       &               & False                            \\
\begin{tabular}[c]{@{}r@{}}Discard patches with more than \\ a \% of zeros in the image\end{tabular}   &                & \textit{choice}[True(50\%), True(80\%), False]      &               & True(50\%)                       \\
Shuffle train on each epoch                                                                            &                & True                                   &               & True                             \\
Data augmentation                                                                                      &                & flips, rotation\_range(180)  &               & flips, rotation\_range(180)\\
Number of epochs                                                                                       &                & \textit{choice}[20, 30, 50, 360]                       &               & 50                               \\
Batch size                                                                                             &                & \textit{choice}[1, 2]                                &               & 1                                \\
Loss type                                                                                              &                &  $\alpha MSE + (1-\alpha)BCE$            &               & $\alpha MSE + (1-\alpha)BCE$       \\
loss weight $\alpha$                                                                                   &                & \textit{choice}[0.9, 0.98]                          &               & 0.98                             \\
Optimizer                                                                                              &                & \textit{choice}[SGD, Adam]                           &               & SGD                              \\
Learning rate                                                                                          &                & \textit{choice}[1e-3, 2e-3]                         &               & 1e-3                             \\
Scheduler                                                                                              &                & \textit{choice}[Reduce on Plateau, OneCycle]        &               & Reduce on Plateau                \\
Patience                                                                                               &                & \textit{choice}[3, 5, 7, 10, 50]                        &               & 7                                \\ \hline
\textbf{Architecture}                                                                                  & \phantom{abc}  & \phantom{abc}                          & \phantom{abc} &                                  \\ \hline
Number of feature maps to start with                                                                   &                & \textit{choice}[32, 64]                              &               & 32                               \\
Dropout type                                                                                           &                & \begin{tabular}[c]{@{}r@{}}Spatial dropout\\ (0.1, 0.1, 0.2, 0.2, 0.3)\end{tabular}&               & \begin{tabular}[c]{@{}r@{}}Spatial dropout\\ (0.1, 0.1, 0.2, 0.2, 0.3)\end{tabular} \\
Pooling type                                                                                           &                & Max-pooling                            &               & Max-pooling                      \\
Kernel initializer                                                                                     &                & he\_normal                              &               & he\_normal                        \\
Activation                                                                                             &                & ELU                                    &               & ELU                              \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{Hyperparameter search space for the proposed Attention Y-Net, first multitask step.}
\end{table}

%%%%%%%%%%%%%%%%%%%%
%% 2nd step table %%
%%%%%%%%%%%%%%%%%%%%

\begin{table}[]
\hspace{-1.4cm}
\begin{adjustbox}{max width=1.22\textwidth}
\begin{tabular}{rcrcr}
\hline
\textbf{Hyperparameter}                                                                                & \phantom{abc}  & \textbf{Search space}                  & \phantom{abc} & \textbf{Best assignment}         \\ \hline
\textbf{Data}                                                                                          & \phantom{abc}  & \phantom{abc}                          & \phantom{abc} & \phantom{abc}                    \\ \hline
Validation                                                                                             &                & True                                   &               & True                             \\
Random validation                                                                                      &                & True                                   &               & True                             \\
\% of train as validation                                                                              &                & 10\%                                   &               & 10\%                             \\
Patches                                                                                                &                & \textit{choice}[Sequential, Random(1000)]           &               & Random(1000)                     \\
Patch size                                                                                             &                & $256\times256$                         &               & $256\times256$                   \\
\begin{tabular}[c]{@{}r@{}}Discard patches with less than \\ a \% of the foreground class\end{tabular} &                & \textit{choice}[True(5\%), True(10\%), False]       &               & False                            \\
\begin{tabular}[c]{@{}r@{}}Discard patches with more than \\ a \% of zeros in the image\end{tabular}   &                & \textit{choice}[True(50\%), True(80\%), False]      &               & True(50\%)                       \\
Shuffle train on each epoch                                                                            &                & True                                   &               & True                             \\
Data augmentation                                                                                      &                & \begin{tabular}[c]{@{}r@{}}flips, rotation\_range(180),\\histogram\_matching(0\%, \\ 25\%, 50\%, 100\%) \end{tabular}  &               & \begin{tabular}[c]{@{}r@{}}flips, rotation\_range(180),\\ histogram\_matching(50\%) \end{tabular}\\
Number of epochs                                                                                       &                & \textit{choice}[15, 20, 30, 40]                        &               & 40                               \\
Batch size                                                                                             &                & 1                                      &               & 1                                \\
Loss type                                                                                              &                & MSE                                    &               & MSE                              \\
Optimizer                                                                                              &                & \textit{choice}[SGD, Adam]                           &               & Adam                              \\
Learning rate                                                                                          &                & \textit{choice}[2e-3, 2e-4]                         &               & 2e-4                             \\
Scheduler                                                                                              &                & \textit{choice}[Reduce on Plateau, OneCycle]        &               & Reduce on Plateau                \\
Patience                                                                                               &                & \textit{choice}[5, 6, 7, 10, 20]                        &               & 6                                \\ \hline
\textbf{Architecture}                                                                                  & \phantom{abc}  & \phantom{abc}                          & \phantom{abc} &                                  \\ \hline
Number of feature maps to start with                                                                   &                & 32                                     &               & 32                               \\
Dropout type                                                                                           &                & \begin{tabular}[c]{@{}r@{}}Spatial dropout\\ (0.1, 0.1, 0.2, 0.2, 0.3)\end{tabular}&               & \begin{tabular}[c]{@{}r@{}}Spatial dropout\\ (0.1, 0.1, 0.2, 0.2, 0.3)\end{tabular} \\
Pooling type                                                                                           &                & Max-pooling                            &               & Max-pooling                      \\
Kernel initializer                                                                                     &                & he\_normal                              &               & he\_normal                        \\
Activation                                                                                             &                & ELU                                    &               & ELU                              \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{Hyperparameter search space for the proposed Attention Y-Net, second step focused in reconstruction.}
\end{table}

%%%%%%%%%%%%%%%%%%%%
%% 3rd step table %%
%%%%%%%%%%%%%%%%%%%%

\begin{table}[]
\hspace{-1.4cm}
\begin{adjustbox}{max width=1.22\textwidth}
\begin{tabular}{rcrcr}
\hline
\textbf{Hyperparameter}                                                                                & \phantom{abc}  & \textbf{Search space}                  & \phantom{abc} & \textbf{Best assignment}         \\ \hline
\textbf{Data}                                                                                          & \phantom{abc}  & \phantom{abc}                          & \phantom{abc} & \phantom{abc}                    \\ \hline
Validation                                                                                             &                & True                                   &               & True                             \\
Random validation                                                                                      &                & True                                   &               & True                             \\
\% of train as validation                                                                              &                & 10\%                                   &               & 10\%                             \\
Patches                                                                                                &                & \begin{tabular}[c]{@{}r@{}}\textit{choice}[Sequential, Random(160,\\ 500, 1000, 2000)]\end{tabular}           &               & Random(1000)                     \\
Patch size                                                                                             &                & $256\times256$                         &               & $256\times256$                   \\
\begin{tabular}[c]{@{}r@{}}Discard patches with less than \\ a \% of the foreground class\end{tabular} &                & \textit{choice}[True(5\%), True(10\%), False]       &               & False                            \\
\begin{tabular}[c]{@{}r@{}}Discard patches with more than \\ a \% of zeros in the image\end{tabular}   &                & \textit{choice}[True(50\%), True(80\%), False]      &               & True(50\%)                       \\
Shuffle train on each epoch                                                                            &                & True                                   &               & True                             \\
Data augmentation                                                                                      &                & \begin{tabular}[c]{@{}r@{}}flips, rotation\_range(180),\\histogram\_matching(0\%, \\25\%, 50\%, 100\%) \end{tabular}  &               & \begin{tabular}[c]{@{}r@{}}flips, rotation\_range(180),\\ histogram\_matching(50\%) \end{tabular}\\
Number of epochs                                                                                       &                & \textit{choice}[5, 10, 20, 100]                        &               & 100                               \\
Batch size                                                                                             &                & 1                                      &               & 1                                \\
Loss type                                                                                              &                & BCE                                    &               & BCE                              \\
Optimizer                                                                                              &                & \textit{choice}[SGD, Adam]                           &               & Adam                              \\
Learning rate                                                                                          &                & \textit{choice}[2e-3, 2e-4]                         &               & 2e-4                             \\
Scheduler                                                                                              &                & \textit{choice}[Reduce on Plateau, OneCycle, None]        &               & oneCycle                \\
Patience                                                                                               &                & \textit{choice}[10, 15, 20, 150]                       &               & 15                                \\ \hline
\textbf{Architecture}                                                                                  & \phantom{abc}  & \phantom{abc}                          & \phantom{abc} &                                  \\ \hline
Number of feature maps to start with                                                                   &                & 32                                     &               & 32                               \\
Dropout type                                                                                           &                & \begin{tabular}[c]{@{}r@{}}Spatial dropout\\ \{0.1, 0.1, 0.2, 0.2, 0.3\}\end{tabular}&               & \begin{tabular}[c]{@{}r@{}}Spatial dropout\\ \{0.1, 0.1, 0.2, 0.2, 0.3\}\end{tabular} \\
Pooling type                                                                                           &                & Max-pooling                            &               & Max-pooling                      \\
Kernel initializer                                                                                     &                & he\_normal                              &               & he\_normal                        \\
Activation                                                                                             &                & ELU                                    &               & ELU                              \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{Hyperparameter search space for the proposed Attention Y-Net, third and last training step, focused in segmentation.}
\end{table}

==> tables/SSL_parameters_table.tex <==
\begin{table}[]
\hspace{-1.4cm}
\begin{adjustbox}{max width=1.22\textwidth}
\begin{tabular}{rcrcr}
\hline
 \textbf{Hyperparameter}                                                                                                                                       &  \phantom{abc} &  \textbf{Search space}                                                                                                                      &  \phantom{abc} &  \textbf{Best assignment}                                                                                                                   \\ \hline
 \textbf{Data}                                                                                                                                                 &  \phantom{abc} &  \phantom{abc}                                                                                                                              &  \phantom{abc} &  \phantom{abc}                                                                                                                              \\ \hline
Validation                                                                                                                                                                     &                                & True                                                                                                                                                        &                                & True                                                                                                                                                        \\
Random validation                                                                                                                                                              &                                & True                                                                                                                                                        &                                & True                                                                                                                                                        \\
\% of train as validation                                                                                                                                                      &                                & 10\%                                                                                                                                                        &                                & 10\%                                                                                                                                                        \\
Patches                                                                                                                                                                        &                                & \begin{tabular}[c]{@{}r@{}} Maximum number that fitted \\ into the slice dimensions  \end{tabular}                     &                                & \begin{tabular}[c]{@{}r@{}} Maximum number that fitted \\ into the slice dimensions  \end{tabular}                     \\
Patch size                                                                                                                                                                     &                                & $256\times256$                                                                                                                                              &                                & $256\times256$                                                                                                                                              \\
  \begin{tabular}[c]{@{}r@{}}Discard patches with less than  \\ a \% of the foreground class \end{tabular} &                                &  \textit{choice}{[}True(2\%),True(5\%), True(10\%), False{]}                                                                      &                                & True(2\%)                                                                                                                                                   \\
Shuffle train on each epoch                                                                                                                                                    &                                & True                                                                                                                                                        &                                & True                                                                                                                                                        \\
Data augmentation                                                                                                                                                              &                                & flips, rotation\_range({[}-180,180,90{]})                                                                                                                   &                                & flips, rotation\_range({[}-180,180,90{]})                                                                                                                   \\
Number of epochs                                                                                                                                                               &                                &  \textit{choice}{[}100,200,300{]}                                                                                                           &                                & 200                                                                                                                                                         \\
Batch size                                                                                                                                                                     &                                &  \textit{choice}{[}1, 2,5{]}                                                                                                                &                                & 1                                                                                                                                                           \\
Loss type                                                                                                                                                                      &                                &  \textit{choice}{[}MAE,MSE{]}                                                                                                               &                                & MAE                                                                                                                                                         \\
Optimizer                                                                                                                                                                      &                                &  \textit{choice}{[}SGD, Adam{]}                                                                                                             &                                & Adam                                                                                                                                                        \\
Learning rate                                                                                                                                                                  &                                &  \textit{choice}{[}1e-3, 2e-3,1e-4,5e-4{]}                                                                                                       &                                & 5e-4                                                                                                                                                        \\
Scheduler                                                                                                                                                                      &                                &  \textit{choice}{[}Reduce on Plateau, OneCycle{]}                                                                                           &                                & OneCycle                                                                                                                                                    \\
Patience                                                                                                                                                                       &                                &  \textit{choice}{[}None,3, 5, 7, 10, 50{]}                                                                                                       &                                & None                                                                                                                                                           \\ \hline
 \textbf{Architecture}                                                                                                                                         &  \phantom{abc} &  \phantom{abc}                                                                                                                              &  \phantom{abc} &                                                                                                                                                             \\ \hline
Number of feature maps to start with                                                                                                                                           &                                & 32                                                                                                                                                          &                                & 32                                                                                                                                                          \\
Dropout type                                                                                                                                                                   &                                &   \begin{tabular}[c]{@{}r@{}}Spatial dropout  (0.1, 0.1, 0.2, 0.2, 0.3) \end{tabular} &                                &   \begin{tabular}[c]{@{}r@{}}Spatial dropout (0.1, 0.1, 0.2, 0.2, 0.3) \end{tabular} \\
Pooling type                                                                                                                                                                   &                                & Max-pooling                                                                                                                                                 &                                & Max-pooling                                                                                                                                                 \\
Kernel initializer                                                                                                                                                             &                                & he\_normal                                                                                                                                                    &                                & he\_normal                                                                                                                                                  \\
Activation                                                                                                                                                                     &                                & ELU                                                                                                                                                         &                                & ELU                                                                                                                                                         \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{ Hyperparameter search space for the proposed self-supervised learning pretraining step
with the Attention U-Net.}

\label{tab:SSLHyper}
\end{table}

\begin{table}[]
\hspace{-1.4cm}
\begin{adjustbox}{max width=1.22\textwidth}
 \begin{tabular}{rcrcr}
\hline
 \textbf{Hyperparameter}                                                                                                                                       &  \phantom{abc} &  \textbf{Search space}                                                                                                                      &  \phantom{abc} &  \textbf{Best assignment}                                                                                                                   \\ \hline
 \textbf{Data}                                                                                                                                                 &  \phantom{abc} &  \phantom{abc}                                                                                                                              &  \phantom{abc} &  \phantom{abc}                                                                                                                              \\ \hline
Validation                                                                                                                                                                     &                                & True                                                                                                                                                        &                                & True                                                                                                                                                        \\
Random validation                                                                                                                                                              &                                & True                                                                                                                                                        &                                & True                                                                                                                                                        \\
\% of train as validation                                                                                                                                                      &                                & 10\%                                                                                                                                                        &                                & 10\%                                                                                                                                                        \\
Patches                                                                                                                                                                        &                                &\begin{tabular}[c]{@{}r@{}} Maximum number that fitted \\ into the slice dimensions  \end{tabular}                    &                                &\begin{tabular}[c]{@{}r@{}} Maximum number that fitted \\ into the slice dimensions  \end{tabular}                     \\
Patch size                                                                                                                                                                     &                                & $256\times256$                                                                                                                                              &                                & $256\times256$                                                                                                                                              \\
  \begin{tabular}[c]{@{}r@{}}Discard patches with less than  \\ a \% of the foreground class \end{tabular} &                                &  \textit{choice}{[}True(2\%),True(5\%), True(10\%), False{]}                                                                      &                                & True(2\%)                                                                                                                                                   \\
Shuffle train on each epoch                                                                                                                                                    &                                & True                                                                                                                                                        &                                & True                                                                                                                                                        \\
Data augmentation                                                                                                                                                              &                                & flips, rotation\_range({[}-180,180,90{]})                                                                                                                   &                                & flips, rotation\_range({[}-180,180,90{]})                                                                                                                   \\
Number of epochs                                                                                                                                                               &                                & {[}10,200,10{]}                                                                                                                                             &                                & 60                                                                                                                                                          \\
Batch size                                                                                                                                                                     &                                & \textit{choice}{[}1, 2,5{]}                                                                                                                &                                & 1                                                                                                                                                           \\
Loss type                                                                                                                                                                      &                                & BCE                                                                                                                                                         &                                & BCE                                                                                                                                                         \\
Optimizer                                                                                                                                                                      &                                & \textit{choice}{[}SGD, Adam{]}                                                                                                             &                                & Adam                                                                                                                                                        \\
Learning rate                                                                                                                                                                  &                                & \textit{choice}{[}1e-3, 2e-3,1e-4{]}                                                                                                       &                                & 1e-4                                                                                                                                                        \\
Scheduler                                                                                                                                                                      &                                & \textit{choice}{[}Reduce on Plateau, OneCycle{]}                                                                                           &                                & OneCycle                                                                                                                                                    \\
Patience                                                                                                                                                                       &                                & \textit{choice}{[}None,3, 5, 7, 10, 50{]}                                                                                                       &                                & None                                                                                                                                                          \\ \hline
 \textbf{Architecture}                                                                                                                                         &  \phantom{abc} &  \phantom{abc}                                                                                                                              &  \phantom{abc} &                                                                                                                                                             \\ \hline
Number of feature maps to start with                                                                                                                                           &                                & 32                                                                                                                                                          &                                & 32                                                                                                                                                          \\
Dropout type                                                                                                                                                                   &                                &   \begin{tabular}[c]{@{}r@{}}Spatial dropout  (0.1, 0.1, 0.2, 0.2, 0.3) \end{tabular} &                                &   \begin{tabular}[c]{@{}r@{}}Spatial dropout (0.1, 0.1, 0.2, 0.2, 0.3) \end{tabular} \\
Pooling type                                                                                                                                                                   &                                & Max-pooling                                                                                                                                                 &                                & Max-pooling                                                                                                                                                 \\
Kernel initializer                                                                                                                                                             &                                & he\_normal                                                                                                                                                   &                                & he\_normal                                                                                                                                                    \\
Activation                                                                                                                                                                     &                                & ELU                                                                                                                                                         &                                & ELU                                                                                                                                                         \\ \hline
\end{tabular}
\end{adjustbox}
\vspace{0.2cm}
\caption{ Hyperparameter search space for the proposed self-supervised learning training step
with the Attention U-Net.}

\label{tab:SSLHyper_train}
\end{table}
